Secondary neutrino and gamma-ray fluxes from SimProp and CRPropa

The interactions of ultra-high-energy cosmic rays (UHECRs) in extragalactic space with photons of the cosmic microwave background (CMB) and extragalactic background light (EBL) can generate high-energy neutrinos and photons. Simulations of UHECR propagation require knowledge about physical quantities such as the spectrum of the EBL and photodisintegration cross sections. These assumptions, as well as the approximations used in the codes, may influence the computed UHECR spectrum and composition, and the associated cosmogenic neutrino and photon fluxes. Following up on our previous work where we studied the effects of these uncertainties on the UHECR spectrum and composition, here we quantify those on neutrino fluxes and production rates of photons, electrons, and positrons, using the Monte Carlo codes CRPropa and SimProp, in various astrophysical scenarios. We show that cosmogenic neutrinos are more sensitive to the choice of EBL model than UHECRs, whereas the overall cosmogenic gamma-ray production rates are relatively independent of propagation details. We also find significant differences between neutrino fluxes predicted by the latest released versions of CRPropa and SimProp, and discuss their causes and possible improvements in future versions of the codes.

==> models_ebl.tex <==
\subsection{EBL models}
\label{sec:EBL}
\AdM{Should this be merged into \sectionref{sec:EBL_comp}?}
Direct observations of the EBL are rather hard due to the presence of a much brighter foreground, the zodiacal light.
Various phenomenological models have been developed to describe its energy spectrum and cosmological evolution adopting different approaches, e.g.~\cite{Kneiske:2003tx,Stecker:2006eh,Franceschini:2008tp,Dominguez:2010bv,Gilmore:2011ks}. Nevertheless, there are sizeable differences even among recent models, especially at long wavelengths and at high redshifts. These were shown~\cite{Batista:2015mea} to result in sizeable differences in predictions of the UHECR spectrum and composition at Earth,
which in turn were shown~\cite{Aab:2016zth} to result in major differences in the injection parameters required
to fit the observed UHECR spectrum and composition data.

In this work, when not otherwise stated we use the Gilmore et~al.~2012~\cite{Gilmore:2011ks} fiducial model (G12).
In a few select cases we also show results using the Dominguez et~al.~2011~\cite{Dominguez:2010bv} best-fit model (D11) for comparison.



==> models_injection.tex <==
\section{The models we used}\label{sec:models}

\subsection{Injection scenarios}\label{sec:injection}
In our comparisons, we used injection scenarios whose spectrum has the form \begin{equation}
	\frac{\mathrm{d}N_\text{inj}}{\mathrm{d}E} \propto \left(\frac{E}{\mathrm{EeV}}\right)^{-\gamma} \exp\left(-\frac{E}{Z\Rcut}\right)
\end{equation} and the source emissivity as a function of the redshift~$z$ is expressed as \begin{align}
	\mathcal{L}(z) = \int_{E_{\min}}^{E_{\max}} \frac{E\,\mathrm{d}N_\text{inj}}{\mathrm{d}E\,\mathrm{d}V_\text{c}\,\mathrm{d}t}\,\mathrm{d}E &= \mathcal{L}_0 S(z), &\begin{aligned} \mathcal{L}(0) &= \mathcal{L}_0, \\ S(0) &= 1,\end{aligned}
\end{align} where $V_\text{c} = (1+z)^3V$ is the comoving volume.
The various combinations of parameters we used are listed in Table~\ref{tab:inj}.
\begin{table}[hbt!]
	\centering
	\caption{The various injection scenarios we considered}
	\label{tab:inj}
	\begin{tabular}{cccccc}
		\hline\hline
		\multirow{2}{*}{name} & \multirow{2}{*}{$^AZ$} & $\mathcal{L}_0$ & \multirow{2}{*}{$S(z)$} & \multirow{2}{*}{$\gamma$} & $\Rcut$ \\
		\cline{3-3} \cline {6-6}
		~ & ~ & $\mathrm{erg}~\mathrm{Mpc}^{-3}~\mathrm{yr}^{-1}$ & ~ & ~ & EV \\
		\hline
		unif.~protons & $^{\phantom{0}1}$H & $1.5\times 10^{46}$ & 1, $z\le 6$ & $2.6$ & $10^{4}$ \\
		SFR~protons & $^{\phantom{00}}$'' & $6.0\times 10^{45}$ & $S_\text{SFR}(z)$ & $2.5$ & '' \\
		AGN~protons & $^{\phantom{00}}$'' & $3.5\times 10^{45}$ & $S_\text{AGN}(z)$ & $2.4$ & '' \\
		hard nitrogen & $^{14}$N & $5.0\times 10^{44}$ & 1, $z\le 6$ & $1.0$ & $5$ \\
		hard iron & $^{56}$Fe & '' & '' & '' & '' \\
		soft nitrogen & $^{14}$N & $1.0\times 10^{45}$ & 1, $z\le 6$ & $2.0$ & $100$ \\
		soft iron & $^{56}$Fe & '' & '' & '' & '' \\
		\hline
	\end{tabular}
	\footnotesize\begin{align*}
		S_\text{SFR}(z) &= \begin{cases}
			(1+z)^{3.4}, & 0 \le z\le 1; \\
			2^{3.7}(1+z)^{-0.3}, & 1 \le z \le 4; \\
			2^{3.7}5^{3.2}(1+z)^{-3.5}, & 4 \le z \le 6.
		\end{cases}& S_\text{AGN}(z) &= \begin{cases}
			(1+z)^5, & 0.0 \le z\le 1.7; \\
			2.7^5, & 1.7 \le z \le 2.7; \\
			2.7^5 10^{2.7-z}, & 2.7 \le z \le 6.0.
		\end{cases}
	\end{align*}
\end{table}
In all cases we took $E_{\min}=10^{16}$~eV, $E_{\max}=10^{23}$~eV, $z_{\min}=0$ and $z_{\max}=6$.

The first three scenarios are based on the ``dip model'' scenarios from Ref.~\cite{Aloisio:2015ega},
but without the spectral break at low energies.
The last four were also used in Ref.~\cite{Batista:2015mea}, and are loosely inspired
to the ``best fit'' and the ``second local minimum'' of Ref.~\cite{Aab:2016zth}.

The proton injection scenarios can approximately reproduce the observed total UHECR spectrum all the way down to $\sim 1~\EeV$,
but heavier elements can only do so above $\sim 5~\EeV$ (the so-called ankle in the UHECR spectrum),
and drastically underestimate it at lower energies.
In order to reasonably describe the spectrum below the ankle, a different origin must be assumed
for most cosmic rays at those energies.
Their observed mass composition is too light and their observed angular distribution is too isotropic \cite{Abbasi:2016kgr}
for their origin to be plausibly Galactic.
Such an additional extragalactic proton population at~$E \lesssim 5~\EeV$ can be presumed to result
in cosmogenic neutrino fluxes $\lesssim 250$~PeV similar to those in proton-only scenarios,
as well as considerable cosmogenic gamma-ray fluxes~\cite{Liu:2016brs}.


==> models_photodis.tex <==
\subsection{Photodisintegration models}\label{sec:disint}
\AdM{Should this be merged into \sectionref{sec:disint_comp}?}
Total photoabsorption cross sections have been measured for 14 nuclides among nuclear isotopes interesting for cosmic-ray astrophysics~\cite{Boncioli:2016lkt}. The experimental situation becomes better if we consider the inclusive cross sections for the emission of neutrons. On the other hand, exclusive cross sections for channels in which all ejected fragments are charged are harder to be measured.
In particular, ${^{A}_{Z}X}(\gamma, \alpha){^{A-4}_{Z-2}X'}$ channels have only been measured for a handful of nuclides. These have a noticeably different impact on UHECR propagation than single-nucleon ejection as the secondaries have four times as much energy.

Phenomenological models to estimate such cross sections are available, but not
necessarily reliable. For instance, TALYS overestimates the exclusive cross section
of ${^{12}\mathrm{C}}(\gamma, \alpha){^{8}\mathrm{Be}}$ by an order of magnitude;
see the Appendix A of Ref.~\cite{Batista:2015mea} and references therein.

In this work, unless otherwise stated, we use photodisintegration cross sections computed using TALYS~\cite{Goriely:2008zu} with parameters restored to those of the preliminary version~\cite{Khan:2004nd}, as described in Ref.~\cite{Batista:2015mea}.
In a few selected cases we also show results using the Puger-Stecker-Bredekamp~\cite{Puget:1976nz} photodisintegration model
with Stecker--Salamon~\cite{Stecker:1998ib} thresholds.


